A continuous energy-based immersed boundary method for elastic shells

The immersed boundary method is a mathematical formulation and numerical method for solving fluid-structure interaction problems. For many biological problems, such as models that include the cell membrane, the immersed structure is a two-dimensional infinitely thin elastic shell immersed in an incompressible viscous fluid. When the shell is modeled as a hyperelastic material, forces can be computed by taking the variational derivative of an energy density functional. A new method for computing a continuous force function on the entire surface of the shell is presented here. The new method is compared to a previous formulation where the surface and energy functional are discretized before forces are computed. For the case of Stokes flow, a method for computing quadrature weights is provided to ensure the integral of the elastic spread force density remains zero throughout a dynamic simulation. Tests on the method are conducted and show that it yields more accurate force computations than previous formulations as well as more accurate geometric information such as mean curvature. The method is then applied to a model of a red blood cell in capillary flow and a 3D model of cellular blebbing.

==> BendingRig.tex <==
\newcommand{\dxodl}{\fraco{\partial X_1}{\partial \lambda}}
\newcommand{\dxtdl}{\fraco{\partial X_2}{\partial \lambda}}
\newcommand{\dxrdl }{\fraco{\partial X_3}{\partial \lambda}}
\newcommand{\dxodt}{\fraco{\partial X_1}{\partial \theta}}
\newcommand{\dxtdt}{\fraco{\partial X_2}{\partial \theta}}
\newcommand{\dxrdt}{\fraco{\partial X_3}{\partial \theta}}
\newcommand{\dsxodldt}{\fraco{\partial^2 X_1}{\partial \lambda \partial \theta}}
\newcommand{\dsxtdldt}{\fraco{\partial^2 X_2}{\partial \lambda \partial \theta}}
\newcommand{\dsxrdldt}{\fraco{\partial^2 X_3}{\partial \lambda \partial \theta}}
\newcommand{\dsxodls}{\fraco{\partial^2 X_1}{\partial \lambda^2}}
\newcommand{\dsxtdls}{\fraco{\partial^2 X_2}{\partial \lambda^2}}
\newcommand{\dsxrdls}{\fraco{\partial^2 X_3}{\partial \lambda^2}}
\newcommand{\dsxodts}{\fraco{\partial^2 X_1}{\partial \theta^2}}
\newcommand{\dsxtdts}{\fraco{\partial^2 X_2}{\partial \theta^2}}
\newcommand{\dsxrdts}{\fraco{\partial^2 X_3}{\partial \theta^2}}

Our method as derived in Section \ref{sec:mathform} can be generalized to forces that depend on the deformed configuration instead of the undeformed one (i.e. the energy functional $W$ gives energy per unit deformed area). Force due to surface tension came from one such energy functional ($W=\sigma$); however in that case simple differential geometry can be used to obtain the expression for force rather than more rigorous variational derivatives \cite{pozrikidis2003modeling}. 
In this section, we present an outline of a general method of computing force from energy densities over the current configuration. We emphasize that this formulation is correct only for functionals that depend on at most one derivative of the position function $\vec{X}$. Consider an energy functional over the deformed state $\Gamma$
\begin{equation}
E= \int_{\Gamma} W \, dA
\end{equation}
Consider once again a deformation by $\delta \vec{X}$. Evaluating Eq.\ \eqref{eq:vardef}:
\begin{equation}
\phi_{\delta \bm{X}}(\alpha) = E(\vec{X} + \alpha \delta \vec{X}) = \int_{\Gamma} W(\mat{\nabla_{\theta}}(\vec{X}+ \alpha \delta \vec{X})) \sqrt{\det{\G}} \, d\lambda \, d\theta
\end{equation}
We begin as before by applying the chain rule for $\mat{\nabla_{\theta} X}$. 
\begin{equation}
\frac{d \phi_{\delta \bm{X}}(\alpha)}{d\alpha}\Bigg|_{\alpha=0} = \sum_{i=1}^3 \sum_{j=1}^2 {\int_{\Gamma} \frac{\partial \left(W \sqrt{\det{\G}}\right)}{\partial (\mat{\nabla_{\theta} X})_{ij}} \frac{\partial \, \delta X_i}{\partial q_j} \, d\lambda \, d\theta}
\end{equation}
Recall that $i$ describes the Cartesian coordinates and is indexed from 1 to 3, $j$ describes the curvilinear coordinates $\lambda$ and $\theta$ and is indexed from 1 to 2. Note that this time the area weight $\sqrt{\det{\G}}$ does depend on the tensor $\mat{\nabla_{\theta} X}$, and therefore must be included in the differentiation. This is the primary difference from the derivation of force in the neo-Hookean case, and it is what makes modeling forces independent of the reference configuration with this method more difficult. 
Applying integration by parts on each of the coordinates $\lambda$ and $\theta$ and assuming the boundary terms cancel out:
\begin{equation}
\frac{d \phi_{\delta \bm{X}}(\alpha)}{d\alpha}\Bigg|_{\alpha=0} = -\sum_{i=1}^3 \sum_{j=1}^2 {\int_{\Gamma} \frac{\partial} {\partial q_j} \left(\frac{\partial \left(W \sqrt{\det{\G}}\right)}{\partial (\mat{\nabla_{\theta} X})_{ij}}  \right) \delta X_i
\, d\lambda \, d\theta}
\end{equation}
We obtain an area integral over the reference configuration by multiplying and dividing by $\sqrt{\det{\Gz}}$,
\begin{equation}
\label{eq:frechsumvd}
\frac{d \phi_{\delta \bm{X}}(\alpha)}{d\alpha}\Bigg|_{\alpha=0} = -\sum_{i=1}^3 \sum_{j=1}^2 {\int_{\Gamma_0}  \frac{1}{\sqrt{\det{\Gz}}}\frac{\partial} {\partial q_j} \left(\frac{\partial \left(W \sqrt{\det{\G}}\right)}{\partial (\mat{\nabla_{\theta} X})_{ij}}\right) \, \delta X_i
dA_0}
\end{equation}
Using the Laplace-Beltrami surface divergence operator in the undeformed state,
\begin{equation}
\label{eq:surfacediva}
\nabla_{\theta} = \frac{1}{\sqrt{\Det{\G_0}}} \left(\frac{\partial}{\partial \lambda} \sqrt{\Det{\G_0}} \textrm{ } \vec{e_1} + \frac{\partial}{\partial \theta} \sqrt{\Det{\G_0}} \textrm{ } \vec{e_2}\right)
\end{equation}
we write the variational derivative from Eq.\ \eqref{eq:frechsumvd} as
\begin{equation}
\label{eq:deldotQ}
\frac{\delta{E}}{\delta \vec{X}} = -\nabla_{\theta} \cdot \ten{Q}^\textrm{T}
\end{equation}
where the tensor $Q$ is given by
\begin{equation}
Q = \frac{\partial \left(W \sqrt{\fraco{\det{\G}}{\det{\Gz}}}\right)}{\partial (\mat{\nabla_{\theta} X})} = \frac{\partial \left(W \sqrt{\det{\C}}\right)}{\partial (\mat{\nabla_{\theta} X})}
\end{equation}
Introducing the surface divergence operator in Eq.\ \eqref{eq:surfacediva} has the effect of an implicit multiplication by $\sqrt{\det{\Gz}}$. This is undone by the division by $\sqrt{\det{\Gz}}$ inside of $\ten{Q}$. The weight $\sqrt{\det{\Gz}}$ can be moved inside the differential operator since it is independent of $\mat{\nabla_{\theta} X}$. It becomes immediately apparent that if $W=\sigma$, then the dot product in Eq.\ \eqref{eq:deldotQ} is the force due to surface tension as derived in Section \ref{sec:surfacetens}.
Using the product rule, $Q$ can be written as:
\begin{equation}
Q^\textrm{T} = \frac{\partial W}{\partial (\mat{\nabla_{\theta} X})^\textrm{T}} \sqrt{\det{\C}} + W\frac{\partial \left(\sqrt{\det{\C}}\right)}{\partial (\mat{\nabla_{\theta} X})^\textrm{T}}
\end{equation}
The second term on the right side is related to the force due to surface tension and can be computed with direct differentiation. In the neo-Hookean case, the first term would be expanded in terms of the Green-Lagrange strain invariants $I_1$ and $I_2$ to yield a simplified solution as shown in Section \ref{sec:forcevariations}.
\newline The force density per unit reference area is therefore, 
\begin{equation}
\vec{F}=-\frac{\delta{E}}{\delta \vec{X}} = \nabla_{\theta} \cdot \ten{Q}^\textrm{T}
\end{equation}
And the force density per unit deformed area becomes,
\begin{equation}
\vec{F_{cur}}= \nabla_{\theta} \cdot \ten{Q}^\textrm{T} \left(\fraco{\det{\Gz}}{\det{\G}}\right)^{1/2}
\end{equation}
This formulation allows us to recover the force per unit deformed density from an energy function given over the deformed configuration. 



